Is It Worth the (Environmental) Cost? Limited Evidence for Temporal Adaptation via Continuous Training

Language is constantly changing and evolving, leaving language models to become quickly outdated. Consequently, we should continuously update our models with new data to expose them to new events and facts. However, that requires additional computing, which means new carbon emissions. Do any measurable benefits justify this cost? This paper looks for empirical evidence to support continuous training. We reproduce existing benchmarks and extend them to include additional time periods, models, and tasks. Our results show that the downstream task performance of temporally adapted English models for social media data do not improve over time. Pretrained models without temporal adaptation are actually significantly more effective and efficient. However, we also note a lack of suitable temporal benchmarks. Our findings invite a critical reflection on when and how to temporally adapt language models, accounting for sustainability.

==> co2_table.tex <==
\begin{table}[!t]
\centering
\begin{tabular}{@{}llc@{}}
\toprule
\textbf{Model} & \multicolumn{1}{l}{\textbf{CO$_2$ (kg)}} & \multicolumn{1}{l}{\textbf{F1}} \\ \midrule
BERTweet\subtt{base} & 0.10 & 63.86 \\
BERTweet\subtt{large} & 0.42 & \textbf{64.55} \\ \midrule
DALM 20-1 &  6.34 & 64.07 \\
DALM 22-3 & \textbf{68.04} & 63.31 \\ \bottomrule
\end{tabular}
\caption{Carbon footprint and downstream performance (F1 macro) on the \textsc{TweetEval} benchmark \citep{barbieri-etal-2020-tweeteval}. DALM 20-1 and 22-2 require, respectively, x15 and x162 consumption of the best-performing model.}
\label{tab:emissions}
\end{table}

==> fact_knowledge.tex <==
\begin{table*}[!t]
\centering
\begin{tabular}{@{}lccccc@{}}
\toprule
\textbf{Model} &  \textbf{Capitals} & \textbf{ConceptNet} & \textbf{Google-RE} & \textbf{SQuAD} & \textbf{T-REx} \\ \midrule
RoBERTa & 34.48 & 15.23 & \textbf{21.77} & 12.46 & \textbf{52.88} \\
%RoBERTa\subtt{large} & \textbf{35.34} & \textbf{18.41} & \textbf{23.73} & \textbf{20.00} & \textbf{58.91} \\
BERTweet\subtt{base} & \textbf{35.34} & 12.57 & 20.30 & 10.16 & 38.92 \\
BERTweet\subtt{large} & 33.62 & \textbf{16.77} & 18.47 & \textbf{16.72} & 51.45 \\
\textit{19-4} & \textit{16.38} & \textit{11.59} & \textit{14.93} & \textit{7.87} & \textit{32.13} \\ \midrule
% 20-1 & +42.11 & +6.23 & -15.60 & +8.33 & +3.20 \\
% 20-2 & +52.63 & +7.69 & -15.85 & +12.50 & +3.60 \\
% 20-3 & +47.37 & +7.80 & -14.62 & +16.67 & +4.72 \\
% 20-4 & +52.63 & +9.26 & -12.78 & +0.00 & +5.20 \\
% 21-1 & +57.90 & +9.32 & -15.85 & +20.83 & +3.29 \\
% 21-2 & +36.84 & +9.67 & -12.90 & +20.83 & +6.23 \\
% 21-3 & +42.11 & +10.72 & -7.13 & +33.33 & +7.97 \\
% 21-4 & +47.37 & +11.71 & -10.20 & +29.17 & +8.38 \\
% 22-1 & +57.90 & +10.89 & -7.25 & +12.50 & +9.21 \\
% 22-2 & +57.90 & +11.94 & -7.00 & +20.83 & +7.64 \\ \bottomrule

20-1 & +6.90 & +0.72 & -2.33 & +0.66 & +1.03 \\
20-2 & +8.62 & +0.89 & -2.37 & +0.98 & +1.16 \\
20-3 & +7.76 & +0.90 & -2.18 & +1.31 & +1.52 \\
20-4 & +8.62 & +1.07 & -1.91 & +0.00 & +1.67 \\
21-1 & +9.48 & +1.08 & -2.37 & +1.64 & +1.06 \\
21-2 & +6.03 & +1.12 & -1.93 & +1.64 & +2.00 \\
21-3 & +6.90 & +1.24 & -1.06 & +2.62 & +2.56 \\
21-4 & +7.76 & +1.36 & -1.52 & +2.30 & +2.69 \\
22-1 & +9.48 & +1.26 & -1.08 & +0.98 & +2.96 \\
22-2 & +9.48 & +1.38 & -1.05 & +1.64 & +2.45 \\ \bottomrule

\end{tabular}
\caption{Accuracy ($\uparrow$) on \textsc{LAMA}. Results of DALMs (20-1 through 22-2) are relative to the first checkpoint (19-4).}
\label{tab:LAMA}
\end{table*}

\subsection{Factual Knowledge Coverage}
\label{ssec:LAMA}

\paragraph{Forgetting}
While changing their internal distributional representations, DALMs can incur different types of ``forgetting''.
\textit{Representational} collapse \citep{aghajanyan2020better} affects models internal representation, worsening its generalization capabilities. New data streams can introduce false facts alongside new events, ``overriding'' previous knowledge and causing \textit{factual} forgetting. \textit{Catastrophic} forgetting \citep{goodfellow2013empirical} is often referred to as the phenomenon caused by further extending training of neural networks. Models trained on one task and then on a second one can lose the ability to solve the former (e.g., DCT can lead to models that fail to fill the blank coherently).

% \begin{itemize}

% \item representational: while the goal of DCT is to adapt to new words and contexts, there are no guarantees that the model preserves its ability to generalize, i.e., leveraging its internal representation to solve downstream tasks. Indeed, weights after adaptation can lead to worse models in downstream tasks; 

% \item factual: the upcoming data collection can introduce false facts alongside new events, possibly overriding previous, correct knowledge;

% \item catastrophic: this phenomenon is a well-known issue caused by further extending training of neural networks \citep{goodfellow2013empirical}. When models are trained on one task, and then on a second one, they can lose the ability to solve the former. In language models, specifically DALMs, DCT can lead to models that fail to fill the blank coherently.\footnote{We refer the reader to Table 6's last row in \citet{loureiro-etal-2022-timelms}, where a recent model completes the sentence \textit{Looking forward to watching <mask> Game tonight!} with \textit{Squid}.}

% \end{itemize}

This paper focuses on the representational and factual aspects and inspects how well DALMs perform in different downstream tasks and how well they retain factual knowledge about the world.
%We leave catastrophic forgetting evaluations to future work.

We tested DALMs on predicting capitals from countries of the world\footnote{Data from \url{https://github.com/tmikolov/word2vec/blob/master/questions-words.txt}} under the form of cloze task (e.g., ``The capital of Morocco is <mask>''), and the more general benchmark LAMA \citep{petroni-etal-2019-language}. The latter is a collection of sentences sampled from four independent knowledge sources, ConceptNet for commonsense knowledge, Google-RE and T-REx about facts from Wikipedia, and the SQuAD question-answering dataset. All LAMA samples are formatted as cloze tasks (e.g., ``The theory of relativity was developed by <mask>'', from SQuAD).

Table~\ref{tab:LAMA} reports performance considering uncased filling accuracy. Results suggest that there is no clear improvement from continuous training. There does not seem to be a clear pattern suggesting that models either learn new things or forget them, bringing additional questions regarding evaluating DALMs. In all tasks, DALMs underperform a pretrained model, being it RoBERTa, BERTweet\subtt{base}, or BERTweet\subtt{large}.

==> stereotypes.tex <==
\subsection{Stereotypical Language}
\label{ssec:stereo}

We measure DALMs perplexity on \textsc{CrowS-Pairs} \citep{nangia-etal-2020-crows} and \textsc{StereoSet} \citep{nadeem-etal-2021-stereoset}, two natural English datasets to measure stereotypes in language models.
Following related work, we use pseudo-perplexity \citep{salazar-etal-2020-masked} to estimate the \textit{probability} that DALMs assign to stereotypical language. Pseudo-perplexity is a common approach to score masked language models. Roughly, it uses the model's MLM score to compute each sentence's (pseudo) log-likelihood as the sum of probabilities assigned to each token when masked, then averages likelihoods over the corpus.

This setup matches \citet{loureiro-etal-2022-timelms}'s, where the authors measure pseudo-perplexity on Twitter data. Here, we study how models react to stereotypical sentences rather than testing generic text. For example, \texttt{``[BLANK] was a new chemist in our lab.''} has a stereotypical resolution if blank-filled with \texttt{``He''} and an anti-stereotypical one with \texttt{``She''}. Recent evidence \citep{nadeem-etal-2021-stereoset} shows that pretrained LMs are less perplexed by the \texttt{``He''} resolution. 
Hence, when adapting LMs over time, we can measure how perplexity is evolving: ideally, we would aim for models to become equally or \textit{less} perplexed by anti-stereotypes than stereotypes.

%Take the sentences ``Women belong to the kitchen.'' and ``Men belong to the kitchen''. Ideally, we would aim for models to become \textit{more} perplexed by the former (the stereotype) and \textit{less} perplexed by the latter. However, new data for DALMs studied in this paper comes from Twitter and a relatively short period: assuming stereotypes cannot be eradicated in such a short time, we can expect to find some in new time frames. In light of that, we rephrase our objective: DALMs should become perplexed by stereotypes as much as (or, ideally, more than) they are by anti-stereotypes.

\begin{table}[!t]
\centering
\begin{tabular}{@{}lccc@{}}
\toprule
\textbf{Model} & \multicolumn{1}{c}{\textbf{Score} $\downarrow$} & \multicolumn{1}{c}{\textbf{S}} & \multicolumn{1}{c}{\textbf{AS}} \\ \midrule
\textit{19-4}                    & \textit{59.68}                     & \textit{61.47}                      & \textit{49.08}                           \\ \midrule
20-1 & -0.77 & -0.24 & -4.67 \\
20-2 & -0.10 & +0.63  & -5.60 \\
20-3 & -0.34 & +0.13  & -3.73 \\
20-4 & +0.34  & +1.46  & -7.48 \\
21-1 & -1.22 & -0.37 & -7.48 \\
21-2 & -2.45 & -1.81 & -6.54 \\
21-3 & -1.56 & -0.55 & -8.41 \\
21-4 & -1.99 & -1.63 & -4.67 \\
22-1 & -2.78 & -1.89 & -9.33 \\
22-2 & -3.22 & -2.90 & -5.60 \\ \bottomrule

% Absolute values
% 20-1 & -0.46 & -0.15 & -2.29 \\
% 20-2 & -0.06 & 0.39 & -2.75 \\
% 20-3 & -0.20 & 0.08 & -1.83 \\
% 20-4 & 0.20 & 0.90 & -3.67 \\
% 21-1 & -0.73 & -0.23 & -3.67 \\
% 21-2 & -1.46 & -1.11 & -3.21 \\
% 21-3 & -0.93 & -0.34 & -4.13 \\
% 21-4 & -1.19 & -1.00 & -2.29 \\
% 22-1 & -1.66 & -1.16 & -4.58 \\
% 22-2 & -1.92 & -1.78 & -2.75 \\ \midrule
% Avg & -0.84 & -0.44 & -3.12 \\ \bottomrule

\end{tabular}
\caption{Performance on \textsc{CrowS-Pairs}. Original dataset metric (Score $\downarrow$) and pseudo-perplexity on stereotypical (\textbf{S}) and anti-stereotypical (\textbf{AS}) samples. Results of diachronic models are relative ($\pm \%$) to the first checkpoint (19-4).}
\label{tab:crowspairs}
\end{table}

\begin{table*}[!th]
\centering
\begin{tabular}{@{}lcccccccc@{}}
\toprule
\textbf{} & \multicolumn{2}{c}{\textbf{Gender}} & \multicolumn{2}{c}{\textbf{Profession}} & \multicolumn{2}{c}{\textbf{Race}} & \multicolumn{2}{c}{\textbf{Religion}} \\
\textbf{Model} & \multicolumn{1}{c}{\textbf{S}} & \multicolumn{1}{c}{\textbf{AS}} & \multicolumn{1}{c}{\textbf{S}} & \multicolumn{1}{c}{\textbf{AS}} & \multicolumn{1}{c}{\textbf{S}} & \multicolumn{1}{c}{\textbf{AS}} & \multicolumn{1}{c}{\textbf{S}} & \multicolumn{1}{c}{\textbf{AS}} \\ \midrule
\textit{19-4} & \textit{30.36} & \textit{52.97} & \textit{64.89} & \textit{80.72} & \textit{44.51} & \textit{58.19} & \textit{23.34} & \textit{43.46} \\ \midrule

20-1 & -12.70 & -8.61 & -12.12 & -19.67 & +0.71 & +7.44 & -12.95 & +22.73 \\
20-2 & -19.46 & -16.52 & -18.50 & -26.03 & -9.68 & +0.51 & -21.75 & +18.40 \\
20-3 & -18.70 & -13.83 & -19.23 & -26.57 & -2.39 & +9.62 & -22.50 & +41.47 \\
20-4 & -16.77 & -13.74 & -22.37 & -27.45 & 0.98 & +16.25 & -23.94 & +43.77 \\
21-1 & -18.01 & -14.29 & -24.92 & -28.50 & -5.98 & +7.92 & -24.38 & +39.12 \\
21-2 & -21.66 & -18.32 & -27.33 & -30.92 & -6.65 & +6.83 & -24.10 & +29.99 \\
21-3 & -22.67 & -18.12 & -29.50 & -33.17 & -10.17 & +2.13 & -24.65 & +29.65 \\
21-4 & -24.49 & -19.78 & -28.95 & -30.70 & -11.42 & -0.58 & -26.85 & +22.16 \\
22-1 & -25.38 & -19.65 & -30.25 & -30.25 & -9.45 & -1.14 & -24.63 & +32.48 \\
22-2 & \textbf{-25.41} & -16.93 & -27.16 & \textbf{-28.68} & \textbf{-10.04} & +3.86 & \textbf{-29.56} & +35.81 \\ \midrule
Avg & -20.52 & -15.98 & -24.03 & -28.19 & -6.41 & +5.28 & -23.53 & 31.56 \\ \midrule \midrule
\textit{19-4} & \textit{9.63} & \textit{8.79} & \textit{13.15} & \textit{20.42} & \textit{11.90} & \textit{12.54} & \textit{6.93} & \textit{7.55} \\ \midrule
20-1 & -15.00 & -1.95 & -16.93 & -18.20 & -8.72 & -9.44 & -10.80 & -6.94 \\
20-2 & -16.17 & -3.73 & -18.66 & -15.01 & -12.73 & -12.31 & -12.89 & -10.39 \\
20-3 & -16.49 & +0.77 & -20.69 & -18.81 & -13.26 & -13.83 & -13.23 & -12.34 \\
20-4 & -14.54 & +0.60 & -20.65 & -17.08 & -13.88 & -14.23 & -14.40 & -12.65 \\
21-1 & -17.43 & -0.09 & -21.33 & -26.45 & -16.88 & -16.50 & -13.99 & -12.60 \\
21-2 & -17.60 & -4.40 & -23.66 & -27.52 & -18.21 & -17.07 & -15.77 & -14.29 \\
21-3 & -19.28 & -3.52 & -26.41 & -31.02 & -20.16 & -19.13 & -16.26 & -15.94 \\
21-4 & -17.76 & -4.21 & -24.77 & -29.26 & -19.89 & -19.47 & -17.06 & -16.25 \\
22-1 & -18.83 & -1.77 & -23.26 & -25.62 & -21.09 & -22.41 & -16.64 & -14.58 \\
22-2 & \textbf{-18.03} & -0.58 & -21.86 & \textbf{-24.70} & -20.73 & \textbf{-21.64} & \textbf{-17.52} & -15.55 \\ \midrule
Avg & -14.68 & -0.92 & -18.64 & -19.39 & -13.97 & -13.95 & -12.88 & -11.27 \\ \bottomrule

% Absolute values
% 20-1 & -3.86 & -4.56 & -7.87 & -15.88 & 0.32 & 4.33 & -3.02 & 9.88 \\
% 20-2 & -5.91 & -8.75 & -12.01 & -21.01 & -4.31 & 0.30 & -5.08 & 8.00 \\
% 20-3 & -5.68 & -7.32 & -12.48 & -21.45 & -1.06 & 5.60 & -5.25 & 18.02 \\
% 20-4 & -5.09 & -7.28 & -14.52 & -22.16 & 0.44 & 9.46 & -5.59 & 19.02 \\
% 21-1 & -5.47 & -7.57 & -16.17 & -23.01 & -2.66 & 4.61 & -5.69 & 17.00 \\
% 21-2 & -6.58 & -9.70 & -17.74 & -24.96 & -2.96 & 3.97 & -5.63 & 13.04 \\
% 21-3 & -6.88 & -9.60 & -19.14 & -26.78 & -4.53 & 1.24 & -5.75 & 12.88 \\
% 21-4 & -7.44 & -10.48 & -18.79 & -24.78 & -5.08 & -0.34 & -6.27 & 9.63 \\
% 22-1 & -7.71 & -10.41 & -19.63 & -24.42 & -4.21 & -0.67 & -5.75 & 14.11 \\
% 22-2 & -7.71 & \textbf{-8.97} & -17.63 & \textbf{-23.15} & \textbf{-4.47} & 2.24 & \textbf{-6.90} & 15.56 \\ \midrule
% Avg & -6.23 & -8.46 & -15.60 & -22.76 & -2.85 & 3.07 & -5.49 & 13.72 \\ \midrule \midrule

% \textit{19-4} & \textit{9.63} & \textit{8.79} & \textit{13.15} & \textit{20.42} & \textit{11.90} & \textit{12.54} & \textit{6.93} & \textit{7.55} \\ \midrule
% 20-1 & -1.44 & -0.17 & -2.23 & -3.72 & -1.04 & -1.18 & -0.75 & -0.52 \\
% 20-2 & -1.56 & -0.33 & -2.45 & -3.06 & -1.52 & -1.54 & -0.89 & -0.78 \\
% 20-3 & -1.59 & 0.07 & -2.72 & -3.84 & -1.58 & -1.73 & -0.92 & -0.93 \\
% 20-4 & -1.40 & 0.05 & -2.72 & -3.49 & -1.65 & -1.78 & -1.00 & -0.95 \\
% 21-1 & -1.68 & -0.01 & -2.81 & -5.40 & -2.01 & -2.07 & -0.97 & -0.95 \\
% 21-2 & -1.69 & -0.39 & -3.11 & -5.62 & -2.17 & -2.14 & -1.09 & -1.08 \\
% 21-3 & -1.86 & -0.31 & -3.47 & -6.33 & -2.40 & -2.40 & -1.13 & -1.20 \\
% 21-4 & -1.71 & -0.37 & -3.26 & -5.97 & -2.37 & -2.44 & -1.18 & -1.23 \\
% 22-1 & -1.81 & -0.16 & -3.06 & -5.23 & -2.51 & -2.81 & -1.15 & -1.10 \\
% 22-2 & \textbf{-1.74} & -0.05 & -2.87 & \textbf{-5.04} & -2.47 & \textbf{-2.71} & \textbf{-1.21} & -1.17 \\ \midrule
% Avg & -0.62 & 0.65 & -1.41 & -2.48 & -0.71 & -0.75 & -0.31 & -0.22 \\ \bottomrule


\end{tabular}
\caption{Pseudo-perplexity on \textsc{StereoSet} intra-sentence (top) and inter-sentence (bottom) CATs divided by target on stereotypical (\textbf{S}) and anti-stereotypical (\textbf{AS}) resolutions. Results of diachronic models are relative to the first checkpoint (19-4). In bold, the resolution (\textbf{A} or \textbf{AS}) the model has become less perplexed by over time.}
\label{tab:stereoset}
\end{table*}

\subsubsection{\textsc{CrowS-Pairs}}
\textsc{CrowS-Pairs} contains 1508 examples of stereotypes common in the United States. Since the authors already provide two distinct sets of stereotypical and anti-stereotypical language, we use them with no changes.

We report pseudo-perplexity and the official score on \textsc{CrowS-Pairs} in Table~\ref{tab:crowspairs}. DALM 19-4 reports an encouraging lower perplexity on anti-stereotypes than stereotypes. On average, perplexity on anti-stereotypes has a steeper decrease than on stereotypes. 
All DALMs improve on the official score compared to 19-4 (the best value is 50), most likely because of the more substantial improvement in anti-stereotypes.
%These results seem to suggest the benefits of DCT to build language models less prone to stereotypes: we double check this claim testing DALMs on a \textsc{StereoSet}, a larger set.

\subsubsection{\textsc{StereoSet}}

\textsc{StereoSet} is a larger dataset composed of almost 17k examples divided into two types of Context Association Tests (CATs), namely intra-sentence and inter-sentence tests. Both categories contain a context sentence and three options the model should choose from to resolve the context.\footnote{A sample intra-sentence CAT has context \texttt{``Girls tend to be more [blank] than boys.''} and options ``soft'', ``determined'', and ``fish''. We refer the reader to \citet{nadeem-etal-2021-stereoset} for further details.} The choice of the model can resolve into a stereotypical, anti-stereotypical, or irrelevant sentence. 

To study pseudo-perplexity on CATs, we verbalize each sample in its three variants.
For intra-sentence CATs, we fill the proposed template and compute pseudo-perplexity on the resulting three sentences. For inter-sentence CATs, we compute pseudo-perplexity on the concatenation between context and each option.

Table~\ref{tab:stereoset} reports our measurements divided by the four targets present in the dataset, namely Gender, Profession, Race, and Religion. Differently from what we observed on \textsc{CrowS-Pairs}, DALM 19-4 is less perplexed by stereotypes in all but one case (inter-sentence CATs on Gender). Also, DALM 22-2 has lower perplexity for stereotypical resolutions of CATs in five cases out of eight, and in two cases (intra-sentence Race and Religion), the model is more perplexed by anti-stereotypes than 19-4. These results contrast those on \textsc{CrowS-Pairs} and pose further questions on the quality of models we are adapting via DCT on Twitter data. 

\subsubsection{Is Perplexity Enough?}

In the previous two sections, we studied pseudo-perplexity on stereotypical language and its trend over time, in many cases a \textit{decreasing} trend. 

However, a decreasing perplexity over time does not necessarily imply that the model will pick up this type of bias to discriminate and ultimately ``do more harm'' in downstream tasks. While the two aspects can be correlated, perplexity is an \textit{intrinsic} measure for which we have limited evidence to correlate with \textit{extrinsic} downstream harm \citep{goldfarb-tarrant-etal-2021-intrinsic,blodgett-etal-2020-language}.  

Nonetheless, perplexity is a proxy for behavior in tasks requiring models to estimate word or sentence probabilities. Low perplexity on stereotypical language causes the model to prefer undesired associations and resolutions, depending on the task \citep{rudinger-etal-2018-gender,nozza-etal-2021-honest}.

We call for a thorough inspection of the dynamics of (pseudo) perplexity beyond general text and in sensitive contexts: new models can adapt to stereotypical language with the risk of consolidating and reinforcing stereotypical beliefs.

==> toxigen_hatecheck.tex <==
\subsection{Implicit Hate Speech Detection and Functional Tests}
\label{ssec:hatespeech}

\begin{table*}[!th]
\centering
\begin{tabular}{@{}lcccccccc@{}}
\toprule
\textbf{Model} &
  \textbf{Muslims} &
  \textbf{Black} &
  \textbf{Disabled} &
  \textbf{Gay} &
  \textbf{Immigrants} &
  \textbf{Trans} &
  \textbf{Women} &
  \multicolumn{1}{l}{\textbf{Avg}} \\ \midrule
\textit{19-4} &
  \textit{\textbf{79.55}} &
  \textit{74.69} &
  \textit{83.26} &
  \textit{73.50} &
  \textit{79.05} &
  \textit{77.32} &
  \textit{79.96} &
  \textit{78.19} \\ \midrule
% 20-1 & -1.82 & 0.28 & -3.23 & 2.22  & 0.55 & 0.84 & \textbf{0.74}  & -0.06 \\
% 20-2 & -1.56 & 0.00  & -2.23 & -1.48 & +0.82  & +0.28 & -1.97 & -0.88 \\
% 20-3 & -1.56 & -0.28 & -1.74 & -2.72 & +1.91  & 0.00 & -2.95 & -1.05 \\
% 20-4 & -2.86 & -0.56 & -2.98 & -2.22 & -1.64 & +0.28 & -2.46 & -1.78 \\
% 21-1 & -2.08 & -0.56 & -3.23 & -1.73 & -1.64 & 0.00 & -0.74 & -1.42 \\
% 21-2 & -2.08 & -0.28 & +0.25  & -1.98 & +1.37  & +0.56 & -0.98 & -0.45 \\
% 21-3 & -0.26 & 0.00  & \textbf{+0.99}  & \textbf{+2.22}  & \textbf{+2.73}  & \textbf{+1.12} & -0.25 & \textbf{+0.94}  \\
% 21-4 & -1.30 & 0.00  & -0.50 & -1.48 & -0.55 & +0.28 & -1.47 & -0.72 \\
% 22-1 & -0.26 & +0.28  & -2.73 & -0.49 & -0.27 & 0.00 & -0.25 & -0.53 \\
% 22-2 & -2.08 & \textbf{+0.56}  & -1.49 & -3.21 & -0.82 & +0.56 & -1.23 & -1.10 \\ \midrule 
% Avg & -1.58 & -0.06 & -1.69 & -1.09 & +0.25 & +0.39 &	-1.15 & -0.70 \\ \bottomrule

20-1 & -1.45 & +0.21 & -2.69 & \textbf{+1.63} & +0.43 & +0.65 & \textbf{+0.59} & -0.09 \\
20-2 & -1.24 & 0.00 & -1.86 & -1.09 & +0.65 & +0.22 & -1.57 & -0.70 \\
20-3 & -1.24 & -0.21 & -1.45 & -2.00 & +1.51 & 0.00 & -2.36 & -0.82 \\
20-4 & -2.27 & -0.41 & -2.48 & -1.63 & -1.30 & +0.22 & -1.96 & -1.41 \\
21-1 & -1.65 & -0.41 & -2.69 & -1.27 & -1.30 & 0.00 & -0.59 & -1.13 \\
21-2 & -1.65 & -0.21 & +0.21 & -1.45 & +1.08 & +0.43 & -0.79 & -0.34 \\
21-3 & -0.21 & 0.00 & \textbf{+0.83} & +1.63 & \textbf{+2.16} & \textbf{+0.86} & -0.20 & \textbf{+0.73} \\
21-4 & -1.03 & 0.00 & -0.41 & -1.09 & -0.43 & +0.22 & -1.18 & -0.56 \\
22-1 & -0.21 & +0.21 & -2.27 & -0.36 & -0.22 & 0.00 & -0.20 & -0.44 \\
22-2 & -1.65 & \textbf{+0.41} & -1.24 & -2.36 & -0.65 & +0.43 & -0.98 & -0.86 \\ \midrule
Avg & -1.26 & -0.04 & -1.41 & -0.80 & +0.19 & +0.30 & -0.92 & -0.56 \\ \bottomrule

\end{tabular}
\caption{Accuracy performance ($\uparrow$) on \textsc{HateCheck} split by target group. Results of diachronic models are relative to the first checkpoint (19-4). Best model per group in bold.}
\label{tab:hatecheck}
\end{table*}

As models are exposed to new social media data, exploring how their representation change towards hateful and stereotypical language is another interesting direction. We hence test DALMs in the task of Hate Speech Detection.
%Technically, while they may be exposed to new forms of hatred online, we do not know how pretraining on those affects downstream generalizability.

Hate speech detection models suffer from lexical overfitting to specific identity terms, flagging texts that explicitly mention them as toxic if they are not \citep{10.1145/3278721.3278729,kennedy-etal-2020-contextualizing}. To avoid this type of technical bias, we fine-tune DALMs on \textsc{ToxiGen}, a large-scale synthetic corpus with \textit{implicit} statements about targets \citep{hartvigsen-etal-2022-toxigen}. The dataset consists of 274k sentences balanced between toxic and benign comments directed to thirteen target groups. 

Next, we test fine-tuned models on the \textsc{HateCheck} benchmark \citep{rottger-etal-2021-hatecheck}. The suite consists of a wide range of functional tests. They are constructed by either slot-filling templated sentences such as \texttt{``I hate [IDENTITY]''} or using spurious clues that can fool the models. Templated sentences use identity terms that refer to seven social groups: Muslims, Black, disabled, gay, immigrants, transgender people, and women.

Table~\ref{tab:hatecheck} reports results on \textsc{HateCheck} split by target group. All but one DALMs show worse performance than the 19-4 reference checkpoint. DALM 21-3 is the best-performing model with the greatest improvements in the categories Gay (+2.2\%), Immigrants (+2.7\%), and Transgender (+1.1\%).
However, we cannot find a trend over time: after nine months' worth of DCT, the model is worse (-1.8\% on average). After nine more months, it is better (+0.9\%), and nine months later, it is worse again (-1.1\%). What happens between 21-3 and 22-2 is of particular interest: the 21-3 DCT is the ``winning'' checkpoint; however, this ``winning'' update is lost and never recovered as early as the next run.
These results show that DCT is not beneficial for downstream performance on the task of Hate Speech Detection, further suggesting that the updated models can lose some of their representational capacity.
